Step in Tine: Forking Processes in Functional Choreographies

Choreographic programming allows a concurrent programmer to write one centralized program and compile it to individual programs for each system participant. This approach simplifies critical properties like deadlock freedom, but it complicates forking new processes, a core concurrent primitive. This work addresses that gap with the choreographic fork calculus $\lambda{\pitchfork}$, the first functional choreographic language with process spawning. $\lambda{\pitchfork}$ provides a deadlock-freedom guarantee while allowing programs to dynamically determine when to spawn new processes, what they will do, and who will communicate with them. All results are formalized in Lean.

==> macros.tex <==
\newcounter{numlevels}
\makeatletter
\NewDocumentCommand{\newMLP}{sO{l}mO{0}om}{
  \IfBooleanTF{#1}{
    \IfValueTF{#5}{
      \WithSuffix\newcommand#3*[#4][#5]
    }{
      \WithSuffix\newcommand#3*[#4]
    }
  }{
    \IfValueTF{#5}{
      \newcommand{#3}[#4][#5]
    }{
      \newcommand{#3}[#4]
    }
  }
  {\ifthenelse{\value{numlevels} > 0}{\begin{array}[t]{@{}#2@{}}}{\begin{array}{#2}}\addtocounter{numlevels}{1}#6\addtocounter{numlevels}{-1}\end{array}}
}
\makeatother

\usepackage{trimspaces}
\makeatletter
\newcommand{\newcommenter}[3]{\ifdraft
    \newcommand{#1}[1]{      \begingroup\small\sffamily\color{#2}        [#3: \trim@spaces{##1}]      \endgroup    }\else
    \newcommand{#1}[1]{\ignorespaces}
  \fi
}
\makeatother
\definecolor{darkgreen}{rgb}{0,0.7,0}
\definecolor{ashley-blue}{rgb}{0.2, 0, 0.9}

\newcommenter{\akh}{purple}{AKH}
\newcommenter{\ethan}{darkgreen}{Ethan}
\newcommenter{\ashley}{ashley-blue}{Ashley}

\definecolor{diffred}{rgb}{1.0, 0.64, 0.64}
\definecolor{diffgreen}{rgb}{0.46, 1.0, 0.55}
\colorlet{diffyellow}{Goldenrod!50}

\newcommand{\diff}[3]{\ifdraft
    \sethlcolor{#1}\hl{#2}  \else    #3  \fi}
\newcommand{\remdiff}[1]{\diff{diffred}{#1}{\ignorespaces}}
\newcommand{\adddiff}[1]{\diff{diffgreen}{#1}{#1}}
\newcommand{\chngdiff}[1]{\diff{diffyellow}{#1}{#1}}

\newcommand{\mathdiff}[3]{\ifdraft
    \mathchoice{\colorbox{#1}{$\displaystyle#2$}}
               {\colorbox{#1}{$\textstyle#2$}}
               {\colorbox{#1}{$\scriptstyle#2$}}
               {\colorbox{#1}{$\scriptscriptstyle#2$}}
  \else    #3  \fi}
\newcommand{\mathremdiff}[1]{\mathdiff{diffred}{#1}{}}
\newcommand{\mathadddiff}[1]{\mathdiff{diffgreen}{#1}{#1}}

\newlength{\localparindent}
\newcommand{\diffbox}[3]{\ifdraft
    \setlength{\localparindent}{\parindent}
    \begin{tcolorbox}[breakable, width=\linewidth, sharp corners=all, boxrule=-4pt, boxsep=-6pt, colback=#1]
      \setlength{\parindent}{\localparindent}      #2    \end{tcolorbox}\else
    #3\fi
}
\newcommand{\remdiffbox}[1]{\diffbox{diffred}{#1}{\ignorespaces}}
\newcommand{\adddiffbox}[1]{\diffbox{diffgreen}{#1}{#1}}

\definecolor{orangeGold}{rgb}{0.67, 0.33, 0.1}
\definecolor{blueViolet}{rgb}{0.54, 0.17, 0.89}
\definecolor{ChorBlue}{HTML}{0053A9}
\definecolor{LocalGreen}{HTML}{007C21}
\definecolor{NtwkRed}{HTML}{E44223}
\definecolor{ChoiceYellow}{HTML}{BB7A00}

\colorlet{chorcolor}{ChorBlue}
\colorlet{localcolor}{LocalGreen}
\colorlet{ntwkcolor}{RedOrange}
\colorlet{choicecolor}{ChoiceYellow}

\definecolor{loccolor}{HTML}{b51963}


\SetRuleLabelVCenter
\newcommand{\DefineNtwkRule}[3]{\DefineRule[N#1Rule]{N-#1}{#2}{#3}}
\newcommand{\DefineChorRule}[3]{\DefineRule[C#1Rule]{C-#1}{#2}{#3}}
\newcommand{\DefineKindingRule}[3]{\DefineRule[K#1Rule]{K-#1}{#2}{#3}}
\newcommand{\DefineTypingRule}[3]{\DefineRule[T#1Rule]{T-#1}{#2}{#3}}
\newcommand{\DefineSpawnRule}[3]{\DefineRule[S#1Rule]{S-#1}{#2}{#3}}

\newlength{\vertrulegap}
\setlength{\vertrulegap}{4pt}

\newcommand{\programfont}[1]{\ensuremath{\mathsf{#1}}\xspace}
\mathchardef\mhyphen="2D
\newcommand{\colrel}[2]{\mathrel{\color{#1}#2}}
\makeatletter
\def\subst@inner#1#2#3\_nil{#1 \mapsto #2\ifx\relax#3\relax\else,\mkern2mu\subst@inner#3\_nil\fi}\newcommand{\raw@subst}[3]{
  \mathchoice{#1{\left[#2\subst@inner#3\_nil\right]}}
             {#1[#2\subst@inner#3\_nil]}
             {#1[#2\subst@inner#3\_nil]}
             {#1[#2\subst@inner#3\_nil]}}
\newcommand{\subst}[3]{\raw@subst{#1}{}{{#2}{#3}}}
\WithSuffix\newcommand\subst*[2]{\raw@subst{#1}{}{#2}}
\newcommand{\hsubst}[4]{\raw@subst{#1}{#2|}{{#3}{#4}}}
\WithSuffix\newcommand\hsubst*[3]{\raw@subst{#1}{#2|}{#3}}
\makeatother

\makeatletter
\newcommand{\narrowfill@}[5]{$\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
  \relax#5#1\mkern-7mu\cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
  \mkern-5mu   #4  \mkern-5mu \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
  \mkern-7mu#3$}
\newcommand{\nRightarrowfill@}{\narrowfill@\Relbar\Relbar\Rightarrow\neq
}
\newcommand*{\xnRightarrow}[2][]{  \ext@arrow 0359\nRightarrowfill@{#1}{#2}}
\makeatother

\makeatletter
\DeclareFontEncoding{LS2}{}{\noaccents@}
\DeclareFontSubstitution{LS2}{stix}{m}{n}
\DeclareSymbolFont{stix@largesymbols}{LS2}{stixex}{m}{n}
\SetSymbolFont{stix@largesymbols}{bold}{LS2}{stixex}{b}{n}
\DeclareMathDelimiter{\lBrace}{\mathopen}{stix@largesymbols}{"E8}{stix@largesymbols}{"0E}
\DeclareMathDelimiter{\rBrace}{\mathclose}{stix@largesymbols}{"E9}{stix@largesymbols}{"0F}
\makeatother

\makeatletter
\NewDocumentCommand{\smallbar}{}{  \mathrel{\mathpalette\smallbar@\relax}}

\newcommand{\current@math@font}[1]{\ifx#1\displaystyle\textfont\else
  \ifx#1\textstyle\textfont\else
  \ifx#1\scriptstyle\scriptfont\else
  \scriptscriptfont\fi\fi\fi
}
\newcommand{\smallbar@factor}[1]{\ifx#1\displaystyle 1.135\else
  \ifx#1\textstyle 1.128\else
  \ifx#1\scriptstyle 1.09\else
  1.06\fi\fi\fi
}

\newcommand{\smallbar@}[2]{\begingroup
  \sbox\z@{$\m@th#1\mapstochar$}\dimen0=\smallbar@factor{#1}\ht\z@
  \dimen2=\dimeval{2\fontdimen22\current@math@font{#1} 2 - \dimen0}  \mbox{$\m@th#1\mkern1mu
    \begin{picture}(0,\dimen0)
    \roundcap
    \linethickness{\fontdimen8\current@math@font{#1}3}
    \Line(0,\dimen2)(0,\dimen0)
    \end{picture}    \mkern1mu$  }\endgroup
}
\makeatother

\makeatletter
\def\def@block@inner#1#2#3\_nil{#1 & #2\ifx\relax#3\relax\else \\ \def@block@inner#3\_nil\fi}\newcommand{\typeset@def@block}[2]{\begin{array}[t]{@{}l@{{}#1{}}l@{}}\def@block@inner#2\_nil\end{array}}
\makeatother

\newcommand{\locKnd}{*_\Loc}
\newcommand{\setKnd}{*_\LocSet}
\newcommand{\finsetKnd}{*_\FinLocSet}
\newcommand{\ty}{\mkern2mu{:}\mkern2mu}
\newcommand{\knd}{\mkern2mu{::}\mkern2mu}
\newcommand{\proves}{\vdash}
\newcommand{\provesrev}{\dashv}
\newcommand{\provesPlus}{\vdash^{\mkern-3mu\scriptscriptstyle+}}
\newcommand{\nproves}{\nvdash}
\newcommand{\eproves}{\Vdash}
\newcommand{\dom}[1]{\operatorname{dom}({#1})}
\newcommand{\seqfun}{\mathrel{\fatsemi}}
\newcommand{\sendsto}{\rightsquigarrow}
\newcommand{\tpat}{\raisebox{1pt}{\footnotesize\ensuremath{@}}}
\newcommand{\namedlocs}[1]{\operatorname{NL}({#1})}
\newcommand{\namedlocsinf}[1]{\operatorname{NL}^\anyLoc({#1})}
\newcommand{\spawnedlocs}[1]{\operatorname{SL}({#1})}
\newcommand{\nl}[1]{\namedlocs{#1}}
\newcommand{\nlinf}[1]{\namedlocsinf{#1}}
\newcommand{\rl}[2][\ctx]{\operatorname{RL}({#1};{#2})}
\newcommand{\fv}[2][]{\operatorname{fv}\if\relax\detokenize{#1}\relax\else_{#1}\fi({#2})}
\newcommand{\height}[1]{\operatorname{height}({#1})}
\newcommand{\maybelessthan}{\preceq_\bot}
\newcommand{\lessthan}[1][]{\preceq_{#1}}
\newcommand{\greaterthan}{\succeq}
\newcommand{\dpbsim}{\mathbin{\underline{\leftrightarrow}_b^\Delta}}
\newcommand{\lessthanabove}{\mathbin{\rotatebox[origin=c]{270}{$\greaterthan$}}}
\newcommand{\lessthanbelow}{\mathbin{\rotatebox[origin=c]{270}{$\lessthan$}}}
\newcommand{\lessthansim}{\precsim}
\newcommand{\greaterthansim}{\succsim}
\newcommand{\lessthansimabove}{\mathbin{\rotatebox[origin=c]{270}{$\greaterthansim$}}}
\newcommand{\lessthansimbelow}{\mathbin{\rotatebox[origin=c]{270}{$\lessthansim$}}}
\newcommand{\iotasync}[1]{\iota\text{sync}_{#1}}
\newcommand{\ntwkmerge}{\sqcup}
\newcommand{\maybentwkmerge}{\sqcup_\bot}
\newcommand{\question}{\text{?}}
\newcommand{\val}[1]{\operatorname{Val}({#1})}
\newcommand{\Undef}{\text{undefined}}
\newcommand{\disj}{~\text{disjoint}}

\newcommand\catMaybes{\programfont{catMaybes}}
\newcommand\doubleplus{+\kern-1.3ex+\kern0.8ex}
\newcommand{\size}[1]{\lvert {#1} \rvert}

\NewEnviron{alignbreak}{\begingroup
  \allowdisplaybreaks
  \begin{align*}
    \BODY
  \end{align*}
  \endgroup
}



\newcommand{\Nec}{\square}
\newcommand{\Pos}{\lozenge}
\newcommand{\Merge}{\sqcup}

\newcommand{\defeq}{\triangleq}
\newcommand{\ifText}{\text{if}~}
\newcommand{\andText}{~\text{and}~}
\newcommand{\orText}{~\text{or}~}
\newcommand{\elseText}{~\text{else}~}
\newcommand{\thenText}{~\text{then}~}
\newcommand{\owText}{\text{otherwise}}

\newMLP*[@{}l@{}]{\Newline}[2]{#1 \\ #2}

\newcommand{\say}[1]{\ensuremath{\LocalColor{\lceil}#1\LocalColor{\rfloor}}}
\newcommand{\quoteto}{\ensuremath{\mathrel{\LocalColor{\say{\mathord{\to}}}}}}

\newcommand{\Locations}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\SysLocs}{\ensuremath{\Omega}\xspace}
\newcommand{\freshLoc}{\text{freshLoc}}
\newcommand{\anyLoc}{\top}

\newcommand{\Int}{\programfont{int}}
\newcommand{\String}{\programfont{string}}
\newcommand{\Bool}{\programfont{bool}}
\newcommand{\Unit}{\programfont{unit}}
\newcommand{\Typ}{\programfont{tyRep}}
\newcommand{\Loc}{\programfont{loc}}
\newcommand{\LocSet}{\programfont{lset}}
\newcommand{\FinLocSet}{\programfont{flset}}
\newcommand{\Empty}{\ensuremath{\mathbf{0}}}
\newcommand{\arr}[1]{\xrightarrow{#1}}
\newcommand{\allty}[3]{\forall {#1}[{#2}] \ldotp {#3}}
\newcommand{\isSum}[3]{\text{isSum}({#1},{#2},{#3})}
\newcommand{\getCase}{\mathrm{getCase}}

\newcommand{\metaInl}{\operatorname{inl}}
\newcommand{\metaInr}{\operatorname{inr}}

\definecolor{orangeGold}{HTML}{AB541A}
\newcommand{\ChoiceCol}[1]{{\color{choicecolor}#1}}
\newcommand{\FontChoice}[1]{\ensuremath{\mathbf{\ChoiceCol{#1}}}\xspace}
\newcommand{\Left}{\FontChoice{L}}
\newcommand{\Right}{\FontChoice{R}}

\newcommand{\LocalCol}[1]{{\color{localcolor}#1}}

\newcommand{\ChorCol}[1]{{\color{chorcolor}#1}}

\newcommand{\FontChoreo}[1]{\programfont{\ChorCol{#1}}}
\newcommand{\seq}{\mathrel{\ChorCol{;}}}
\newcommand{\ColSend}{\mathrel{\ChorCol{\sendsto}}}
\newcommand{\ColGive}{\mathrel{\ChorCol{\givesto}}}
\newcommand{\NtwkSend}{\mathrel{\NtwkCol{\sendsto}}}
\newcommand{\ChorSend}[1][\ell]{\mathrel{\mathchoice{\raisebox{0.15ex}{$\scriptstyle\ChorCol{\{}#1\ChorCol{\}}$}\mkern-2mu\ChorCol{\sendsto}}
  {\raisebox{0.15ex}{$\scriptstyle\ChorCol{\{}#1\ChorCol{\}}$}\mkern-2mu\ChorCol{\sendsto}}
  {\mkern3mu\raisebox{0.1ex}{$\scriptstyle\ChorCol{\{}#1\ChorCol{\}}$}\mkern-1mu\ChorCol{\sendsto}}
  {\mkern3mu\raisebox{0.05ex}{$\scriptstyle\ChorCol{\{}#1\ChorCol{\}}$}\mkern-1mu\ChorCol{\sendsto}}}}
\newcommand{\syncs}[3]{{#1}\ChorCol{[}{#2}\ChorCol{]} \mathrel{\ChorCol{\sendsto}} {#3}}
\newcommand{\LetN}{\FontChoreo{let}}
\newcommand{\In}{\FontChoreo{in}}
\newcommand{\IfN}{\FontChoreo{if}}
\newcommand{\ThenN}{\FontChoreo{then}}
\newcommand{\ElseN}{\FontChoreo{else}}
\newcommand{\FunN}{\FontChoreo{fun}}
\newcommand{\TFunN}{\FontChoreo{tfun}}
\newcommand{\TLamN}{\ChorCol{\Lambda}}
\newcommand{\ChorDef}{\mathrel{\ChorCol{\coloneqq}}}
\newcommand{\TellN}{\FontChoreo{tell}}
\newcommand{\To}{\FontChoreo{to}}
\newcommand{\InlN}{\FontChoreo{inl}}
\newcommand{\InrN}{\FontChoreo{inr}}
\newcommand{\LocalInlN}{\LocalLangFont{inl}}
\newcommand{\LocalInrN}{\LocalLangFont{inr}}
\newcommand{\FstN}{\FontChoreo{fst}}
\newcommand{\SndN}{\FontChoreo{snd}}
\newcommand{\FoldN}{\FontChoreo{fold}}
\newcommand{\UnfoldN}{\FontChoreo{unfold}}
\newcommand{\MapN}{\programfont{map}}
\newcommand{\ForkN}{\FontChoreo{fork}}
\newcommand{\KillN}{\FontChoreo{kill}}
\newcommand{\AfterN}{\FontChoreo{after}}
\newcommand{\KillAfterN}{\ensuremath{\operatorname{\FontChoreo{kill-after}}}\xspace}
\newcommand{\LamN}{\ChorCol{\lambda}}
\newcommand{\CaseN}{\FontChoreo{case}}
\newcommand{\LocalCaseN}{\FontChoreo{localCase}}
\newcommand{\OfN}{\FontChoreo{of}}

\newcommand{\LetIn}[3]{\LetN~{#1} \ChorDef {#2}~\In~{#3}}
\newMLP*[r@{~}l]{\LetIn}[3]{\LetN & {#1} \ChorDef {#2} \\ \In & {#3}}
\newMLP*{\LetInLine}[3]{\LetN~{#1} \ChorDef {#2}~\In \\ {#3}}
\makeatletter
\newMLP{\LetMany}[2]{\LetN ~ {\typeset@def@block{\ChorDef}{#1}} \\ \In ~ {#2}}
\makeatother
\newcommand{\ITE}[4][\rho]{\IfN_{#1}~{#2}~\ThenN~{#3}~\ElseN~{#4}}
\newMLP*{\ITE}[4][\rho]{\IfN_{#1}~{#2} \\ \ThenN~{#3} \\ \ElseN~{#4}}
\newcommand{\ITEBase}[3]{\IfN~{#1}~\ThenN~{#2}~\ElseN~{#3}}
\newMLP*{\ITEBase}[3]{\IfN~{#1} \\ \ThenN~{#2} \\ \ElseN~{#3}}
\newcommand{\Fun}[4]{\operatorname{\FunN}_{#1}{#2}({#3}) \ChorDef {#4}}
\newMLP*{\Fun}[4]{\operatorname{\FunN}_{#1}{#2}({#3}) \ChorDef \\ {#4}}
\newcommand{\FunAnnot}[5]{\operatorname{\FunN}_{#1}{#2}({#3}) \ty {#4} \ChorDef {#5}}

\newcommand{\TLam}[2]{\TLamN{#1}\ChorCol{\ldotp{}} {#2}}
\newcommand{\TFun}[4]{\operatorname{\TFunN}_{#1}{#2}({#3}) \ChorDef {#4}}
\newcommand{\TFunLoc}[3]{\operatorname{\TFunN}{#1}({#2}) \ChorDef {#3}}
\newcommand{\TFunAnnot}[5]{\operatorname{\TFunN}_{#1}{#2}({#3}) \ty {#4} \ChorDef {#5}}
\newcommand{\Inl}[2]{\InlN_{#1}~{#2}}
\newcommand{\Inr}[2]{\InrN_{#1}~{#2}}
\newcommand{\Case}[6]{\CaseN_{#1}~{#2}~\FontChoreo{of}~(\InlN~{#3}\Rightarrow{#4})~(\InrN~{#5}\Rightarrow{#6})}
\newMLP*{\Case}[6]{\CaseN_{#1}~{#2}~\FontChoreo{of} \\ \mid \InlN~{#3}\Rightarrow{#4} \\ \mid \InrN~{#5}\Rightarrow{#6}}
\newcommand{\LocalCase}[6]{\LocalCaseN_{#1}~{#2}~\FontChoreo{of}~(\LocalInlN~{#3}\Rightarrow{#4})~(\LocalInrN~{#5}\Rightarrow{#6})}
\newMLP*{\LocalCase}[6]{\LocalCaseN_{#1}~{#2}~\FontChoreo{of} \\ {}\mid \LocalInlN~{#3}\Rightarrow{#4} \\ {}\mid \LocalInrN~{#5}\Rightarrow{#6}}
\newcommand{\LocalCaseBase}[5]{\LocalCaseN~{#1}~\FontChoreo{of}~(\LocalInlN~{#2}\Rightarrow{#3})~(\LocalInrN~{#4}\Rightarrow{#5})}
\newMLP*{\LocalCaseBase}[5]{\LocalCaseN~{#1}~\FontChoreo{of} \\ {}\mid {#2}\Rightarrow{#3} \\ {}\mid {#4}\Rightarrow{#5}}
\newcommand{\Fst}[2]{\FstN_{#1}~{#2}}
\newcommand{\Snd}[2]{\SndN_{#1}~{#2}}
\newcommand{\Fold}[2]{\FoldN_{#1}~{#2}}
\newcommand{\Unfold}[2]{\UnfoldN_{#1}~{#2}}
\newcommand{\Fork}[3]{\LetN~{#1}\ChorDef{#2}.\ForkN()~\In~{#3}}
\newMLP*{\Fork}[3]{\LetN~{#1}\ChorDef{#2}.\ForkN() \\ \In~{#3}}
\newcommand{\LetFork}[4]{\LetN~{#1}\ChorDef{#2}.\ForkN()\ColSend{#3}~\In~{#4}}
\newcommand{\KillAfter}[2]{\KillN~{#1}~\AfterN~{#2}}
\newMLP*{\KillAfter}[2]{\KillN~{#1} \\ \AfterN~{#2}}

\newcommand{\app}[1]{\mathbin{\$_{#1}}}
\newcommand{\tyknd}[1]{*_{#1}}

\newcommand{\AppN}{\FontChoreo{\$}}
\newcommand{\NtwkAppN}{\FontNtwk{\$}}
\newcommand{\appchor}[1]{\mathbin{\AppN_{#1}}}
\newcommand{\appntwk}[1]{\mathbin{\NtwkAppN_{#1}}}

\newcommand{\NtwkCol}[1]{{\color{ntwkcolor}#1}}
\newcommand{\FontNtwk}[1]{\ensuremath{\mathtt{\NtwkCol{#1}}}\xspace}
\newcommand{\FontSys}[1]{\ensuremath{\mathtt{#1}}\xspace}

\newcommand{\NtwkDef}{\mathrel{\NtwkCol{\coloneqq}}}
\newcommand{\AmIN}{\FontNtwk{AmI}}
\newcommand{\AmIInN}{\AmIN\mathord{\NtwkCol{\in}}}
\newcommand{\PIDN}{\FontNtwk{pid}}
\newcommand{\NtwkIn}{\FontNtwk{in}}
\newcommand{\NtwkThen}{\FontNtwk{then}}
\newcommand{\NtwkElse}{\FontNtwk{else}}
\newcommand{\NtwkLeft}{\Left}
\newcommand{\NtwkRight}{\Right}
\newcommand{\NtwkFunN}{\FontNtwk{fun}}
\newcommand{\NtwkTFunN}{\FontNtwk{tfun}}
\newcommand{\NtwkInlN}{\FontNtwk{inl}}
\newcommand{\NtwkInrN}{\FontNtwk{inr}}
\newcommand{\NtwkFstN}{\FontNtwk{fst}}
\newcommand{\NtwkSndN}{\FontNtwk{snd}}
\newcommand{\NtwkFoldN}{\FontNtwk{fold}}
\newcommand{\NtwkUnfoldN}{\FontNtwk{unfold}}
\newcommand{\NtwkVal}[1]{\operatorname{Val}({#1})}
\newcommand{\NtwkForkN}{\FontNtwk{fork}}
\newcommand{\NtwkExit}{\FontNtwk{exit}}
\newcommand{\SysForkN}{\FontSys{fork}}
\newcommand{\SysKillN}{\FontSys{kill}}
\newcommand{\NtwkPar}{\mathrel{\NtwkCol{\parallel}}}
\newcommand{\NtwkLetN}{\FontNtwk{let}}
\newcommand{\NtwkInN}{\FontNtwk{in}}
\newcommand{\NtwkIfN}{\FontNtwk{if}}
\newcommand{\NtwkAsN}{\FontNtwk{as}}
\newcommand{\NtwkTLamN}{\NtwkCol{\Lambda}}
\newcommand{\NtwkLamN}{\NtwkCol{\lambda}}

\newcommand{\NtwkLetIn}[3]{\NtwkLetN~{#1} \NtwkDef {#2}~\NtwkInN~{#3}}
\newcommand{\PID}[2]{\PIDN~\NtwkAsN~{#1}~\NtwkInN~{#2}}
\newMLP*[r@{~}l]{\NtwkLetIn}[3]{\NtwkLetN & {#1} \NtwkDef {#2} \\ \NtwkInN & {#3}}
\newMLP*{\NtwkLetInLine}[3]{\NtwkLetN~{#1} \NtwkDef {#2}~\NtwkInN \\ {#3}}
\makeatletter
\newMLP{\NtwkLetMany}[2]{\NtwkLetN ~ {\typeset@def@block{\NtwkDef}{#1}} \\ \NtwkIn ~ {#2}}
\makeatother

\newcommand{\NtwkUnit}{\FontNtwk{()}}
\newcommand{\NtwkNone}{\Undef}
\newcommand{\SendN}{\FontNtwk{send}}
\newcommand{\RecvN}{\FontNtwk{recv}}
\newcommand{\FromN}{\FontNtwk{from}}
\newcommand{\AllowN}{\FontNtwk{allow}}
\newcommand{\ChoiceN}{\FontNtwk{choice}}
\newcommand{\ChooseForN}{\ensuremath{\operatorname{\FontNtwk{choose-for}}}\xspace}
\newcommand{\AllowChoiceN}{\ensuremath{\operatorname{\FontNtwk{allow-choice}}}\xspace}

\newcommand{\Ret}[1]{\FontNtwk{ret}({#1})}
\newcommand{\SendTo}[2]{\SendN~{#1}~\FontNtwk{to}~{#2}}
\newcommand{\RecvFrom}[1]{\RecvN~\FromN~{#1}}
\newcommand{\SendTy}[4]{\SendN~{#1} \NtwkDef {#2}~\FontNtwk{to}~{#3}~\FontNtwk{in}~{#4}}
\newcommand{\RecvTy}[3]{\RecvN~{#1}~\FromN~{#2}~\FontNtwk{in}~{#3}}
\newcommand{\ChooseFor}[3]{\FontNtwk{choose}~{#1}~\FontNtwk{for}~{#2} \NtwkSeq {#3}}
\newcommand{\AllowChoice}[3]{\AllowN~{#1}~\ChoiceN~(\NtwkLeft \Rightarrow {#2}) ~ (\NtwkRight \Rightarrow {#3})}
\newMLP*{\AllowChoice}[3]{\AllowN~{#1}~\ChoiceN \\ \mid \NtwkLeft \Rightarrow {#2} \\ \mid \NtwkRight \Rightarrow {#3}}
\newMLP*{\AllowChoiceFlat}[3]{\AllowN~{#1}~\ChoiceN \\ \mid \NtwkLeft \Rightarrow {#2} ~\mid \NtwkRight \Rightarrow {#3}}
\newcommand{\AllowOneChoice}[3]{\AllowN~{#1}~\ChoiceN~({#2} \Rightarrow {#3})}
\newMLP*{\AllowOneChoice}[3]{\AllowN~{#1}~\ChoiceN \\ \mid {#2} \Rightarrow {#3}}
\newMLP*[@{\mkern2mu}l@{\mkern2mu}]{\AllowChoiceTight}[3]{\AllowN~{#1}~\ChoiceN \\ \mid \NtwkLeft \Rightarrow {#2} \\ \mid \NtwkRight \Rightarrow {#3}}
\newMLP*[@{\mkern2mu}l@{\mkern2mu}]{\AllowOneChoiceTight}[3]{\AllowN~{#1}~\ChoiceN \\ \mid {#2} \Rightarrow {#3}}
\newcommand{\LetRecvIn}[3]{\RecvN~{#1}~\FromN~{#2}~\NtwkIn~{#3}}
\newcommand{\LetSendIn}[4]{\SendN~{#1} \NtwkDef {#2}~\FontNtwk{to}~{#3}~\NtwkIn~{#4}}
\newcommand{\AmI}[3]{\AmIN~{#1}~\NtwkThen~{#2}~\NtwkElse~{#3}}
\newMLP*[r@{~}l]{\AmI}[3]{\AmIN~{#1} & \NtwkThen~{#2} \\ & \NtwkElse~{#3}}
\newcommand{\AmIIn}[3]{\AmIInN~{#1}~\NtwkThen~{#2}~\NtwkElse~{#3}}
\newMLP*[r@{~}l]{\AmIIn}[3]{\AmIInN~{#1} & \NtwkThen~{#2} \\ & \NtwkElse~{#3}}
\newcommand{\NtwkSeq}{\mathrel{\NtwkCol{;}}}
\newcommand{\IAm}[1]{\text{IAmIn}~{#1}}
\newcommand{\NtwkInl}[1]{\NtwkInlN~{#1}}
\newcommand{\NtwkInr}[1]{\NtwkInrN~{#1}}
\newcommand{\NtwkCase}[5]{\FontNtwk{case}~{#1}~\FontNtwk{of}~(\NtwkInl{#2}\Rightarrow{#3})~(\NtwkInr{#4}\Rightarrow{#5})}
\newMLP*{\NtwkCase}[5]{\FontNtwk{case}~{#1}~\FontNtwk{of} \\ \mid \NtwkInl{#2}\Rightarrow{#3} \\ \mid \NtwkInr{#4}\Rightarrow{#5}}
\newcommand{\NtwkLocalCase}[5]{\FontNtwk{localCase}~{#1}~\FontNtwk{of}~(\LocalInl{#2}\Rightarrow{#3})~(\LocalInr{#4}\Rightarrow{#5})}
\newMLP*{\NtwkLocalCase}[5]{\FontNtwk{localCase}~{#1}~\FontNtwk{of} \\ \mid \LocalInl{#2}\Rightarrow{#3} \\ \mid \LocalInr{#4}\Rightarrow{#5}}
\newcommand{\NtwkFst}[1]{\NtwkFstN~{#1}}
\newcommand{\NtwkSnd}[1]{\NtwkSndN~{#1}}
\newcommand{\NtwkFold}[1]{\NtwkFoldN~{#1}}
\newcommand{\NtwkUnfold}[1]{\NtwkUnfoldN~{#1}}
\newcommand{\NtwkFork}[3]{\NtwkLetN~{#1}\NtwkDef\NtwkForkN({#2})~\NtwkIn~{#3}}
\newMLP*{\NtwkFork}[3]{\NtwkLetN~{#1}\NtwkDef\NtwkForkN({#2}) \\ \NtwkIn~{#3}}

\newcommand{\LocalColor}[1]{{\color{localcolor}#1}}
\newcommand{\LocalLangFont}[1]{\programfont{\color{localcolor}#1}}
\newcommand{\True}{\LocalLangFont{true}}
\newcommand{\False}{\LocalLangFont{false}}
\newcommand{\Loop}{\LocalLangFont{loop}}
\newcommand{\List}[1]{\programfont{list}({#1})}
\newcommand{\Chan}[1]{\programfont{chan}({#1})}
\newcommand{\Maybe}[1]{\programfont{maybe}({#1})}
\newcommand{\Some}[1]{\programfont{some}({#1})}
\newcommand{\None}{\programfont{none}}
\newcommand{\LocalInl}[1]{\LocalInlN~{#1}}
\newcommand{\LocalInr}[1]{\LocalInrN~{#1}}
\newcommand{\ChorSome}[1]{\FontChoreo{some}({#1})}
\newcommand{\ChorNone}{\FontChoreo{none}}
\newcommand{\LocalSome}[1]{\LocalLangFont{some}({#1})}
\newcommand{\LocalNone}{\LocalLangFont{none}}
\newcommand{\Nil}{\LocalLangFont{nil}}
\newcommand{\Cons}[2]{\LocalLangFont{cons}({#1},{#2})}
\newcommand{\NtwkFun}[3]{\operatorname{\NtwkFunN} {#1}({#2}) \NtwkDef {#3}}
\newMLP*{\NtwkFun}[3]{\operatorname{\NtwkFunN} {#1}({#2}) \NtwkDef \\ {#3}}
\newcommand{\NtwkTFun}[3]{\operatorname{\NtwkTFunN} {#1}({#2}) \NtwkDef {#3}}
\newMLP*{\NtwkTFun}[3]{\operatorname{\NtwkTFunN} {#1}({#2}) \NtwkDef \\ {#3}}
\newcommand{\LocalBinop}{\mathbin{\LocalLangFont{\otimes}}}
\newcommand{\LocalPlus}{\mathbin{\LocalLangFont{+}}}
\newcommand{\LocalMinus}{\mathbin{\LocalLangFont{-}}}
\newcommand{\LocalTimes}{\mathbin{\LocalLangFont{*}}}
\newcommand{\LocalLess}{\mathrel{\LocalLangFont{<}}}
\newcommand{\LocalLeq}{\mathrel{\LocalLangFont{\leq}}}
\newcommand{\LocalGreater}{\mathrel{\LocalLangFont{>}}}
\newcommand{\LocalEq}{\mathrel{\LocalLangFont{=}}}
\newcommand{\LocalITE}[3]{\LocalLangFont{if}~{#1}~\LocalLangFont{then}~{#2}~\LocalLangFont{else}~{#3}}
\newcommand{\LocalLangCase}[5]{\LocalLangFont{case}~{#1}~\LocalLangFont{of}~({#2} \Rightarrow {#3})~({#4} \Rightarrow {#5})}
\newcommand{\LocalFun}[3]{\operatorname{\LocalLangFont{fun}}{#1}({#2}) \mathrel{\LocalColor{\coloneqq}} {#3}}
\newcommand{\LocalLam}{\LocalLangFont{\lambda}}
\newcommand{\LocalCast}[2]{\LocalLangFont{cast}({#1},{#2})}
\newcommand{\LocalFold}[1]{\LocalLangFont{fold}~{#1}}
\newcommand{\LocalUnfold}[1]{\LocalLangFont{unfold}~{#1}}
\newcommand{\LocalFst}[1]{\LocalLangFont{fst}~{#1}}
\newcommand{\LocalSnd}[1]{\LocalLangFont{snd}~{#1}}

\newcommand\hole{\ensuremath{[\boldsymbol{\cdot}]}}

\newcommand{\LocFont}[1]{\programfont{\color{loccolor}#1}}
\newcommand{\Client}{\LocFont{C}}
\newcommand{\Leader}{\LocFont{L}}
\newcommand{\Worker}{\LocFont{W}}
\newcommand{\Mngr}{\LocFont{M}}
\newcommand{\Alice}{\LocFont{A}}
\newcommand{\Bob}{\LocFont{B}}
\newcommand{\David}{\LocFont{D}}
\newcommand{\Server}{\LocFont{S}}
\newcommand{\Location}{\LocFont{L}}
\newcommand{\LocOne}{\LocFont{L_1}}
\newcommand{\LocTwo}{\LocFont{L_2}}
\newcommand{\RunAtWorker}{\programfont{runAtW}}
\newcommand{\WithWorker}{\programfont{runWithWorker}}
\newcommand{\AcquireWorker}{\LocalLangFont{acqWorker}}
\newcommand{\Pool}{\LocFont{pool}}
\newcommand{\ReleaseWorker}{\LocalLangFont{relWorker}}
\newcommand{\Tasks}{\LocalLangFont{tasks}}
\newcommand{\ParallelSum}{\programfont{parallelMapSum}}
\newcommand{\LocalSum}{\LocalLangFont{sum}}
\newcommand{\Sum}{\programfont{sum}}
\newcommand{\RecursiveSum}{\programfont{recursiveSum}}
\newcommand{\RecursiveSumImpl}{\programfont{recursiveSumImpl}}
\newcommand{\Len}{\LocalLangFont{len}}
\newcommand{\Split}{\LocalLangFont{split}}
\newcommand{\SumAt}{\programfont{sumAt}}
\newcommand{\SumWithWorker}{\programfont{sumWithWorker}}
\newcommand{\ReserveWorkerGood}{\programfont{runThread}}
\newcommand{\ReserveWorkerBad}{\programfont{runThreadBad}}
\newcommand{\ForkChain}{\programfont{forkChain}}
\newcommand{\ForkBomb}{\programfont{forkBomb}}
\newcommand{\SpawnRing}{\programfont{spawnRing}}
\newcommand{\PassRing}{\programfont{passRing}}
\newcommand{\HandleRequest}{\programfont{handleRequest}}
\newcommand{\task}{\programfont{task}}
\newcommand{\XS}{\mathit{XS}}
\newcommand{\xs}{\mathit{xs}}
\newcommand{\MaxLen}{\LocalLangFont{LOCAL\_MAX\_LEN}}
\newcommand{\MergeSort}{\programfont{mergeSort}}
\newcommand{\MergeList}{\LocalLangFont{merge}}
\newcommand{\SmallList}{\LocalLangFont{smallList}}
\newcommand{\SplitA}{\LocalLangFont{split1}}
\newcommand{\SplitB}{\LocalLangFont{split2}}

\theoremstyle{theorem}
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}
\theoremstyle{definition}
\newtheorem{defn}{Definition}
\newtheorem{ex}{Example}
\newtheorem{conj}{Conjecture}

\declaretheorem[style=theorem]{theorem, lemma}

\newcommand{\todo}[1]{\textcolor{red}{TODO}\xspace(\textcolor{red}{#1})}

\newcommand{\lamqc}{\ensuremath{\lambda}\textsc{qc}\xspace}
\newcommand{\pirouette}{Pirouette}
\newcommand{\helamsm}{\rotatebox[origin=c]{15}{\textphnc{e}}\kern-1pt\textsubscript{$\lambda$small}}
\newcommand{\lamfork}{\ensuremath{\lambda}\scaleto{\pitchfork}{5.5pt}\kern-0.5pt\xspace}
\newcommand{\maty}{\textsf{Maty}\xspace}

\newcommand\proj[2]{\ensuremath{\left.#1\right|_{#2}}}

\newcommand{\epp}[2]{\mathchoice{\left\llbracket#1\right\rrbracket_{#2}}
  {\llbracket#1\rrbracket_{#2}}
  {\llbracket#1\rrbracket_{#2}}
  {\llbracket#1\rrbracket_{#2}}}

\newcommand{\eppfork}[2]{\mathchoice{\left\llbracket#1\right\rrbracket^\pitchfork_{#2}}
  {\llbracket#1\rrbracket^\pitchfork_{#2}}
  {\llbracket#1\rrbracket^\pitchfork_{#2}}
  {\llbracket#1\rrbracket^\pitchfork_{#2}}}

\newcommand{\tbodies}[2]{\mathchoice{\text{tbodies}\left(#1\right)_{#2}}
  {\text{tbodies}(#1)_{#2}}
  {\text{tbodies}(#1)_{#2}}
  {\text{tbodies}(#1)_{#2}}}

\newcommand{\eppall}[1]{\mathchoice{\left\llbracket#1\right\rrbracket}
  {\llbracket#1\rrbracket}
  {\llbracket#1\rrbracket}
  {\llbracket#1\rrbracket}}
\newcommand{\eppnone}[1]{\mathchoice{\left\llbracket#1\right\rrbracket}
  {\llbracket#1\rrbracket}
  {\llbracket#1\rrbracket}
  {\llbracket#1\rrbracket}}

\newcommand{\conf}[2]{\mathchoice{\left\langle {#1}, {#2} \right\rangle}
  {\langle {#1}, {#2} \rangle}
  {\langle {#1}, {#2} \rangle}
  {\langle {#1}, {#2} \rangle}}
\WithSuffix\newcommand\conf*[1]{\conf{#1}{\Omega}}
\makeatletter
\newlength{\@overset@width}
\newcommand{\raw@step}[3]{\mathrel{\if\relax\detokenize{#1}\relax
    \Longrightarrow
  \else
    \setbox0=\hbox{$\scriptstyle#1$}\setlength{\@overset@width}{\wd0}
    \ifdim\@overset@width<0.75em
      {\mathchoice{\overset{#1\mkern4mu}{\Longrightarrow}}
                  {\overset{\raisebox{-1.5pt}[0pt][0pt]{$\scriptstyle#1$}\mkern4mu}{\Longrightarrow}}
                  {\overset{#1\mkern4mu}{\Longrightarrow}}
                  {\overset{#1\mkern4mu}{\Longrightarrow}}}{}
    \else
      {\mathchoice{\xRightarrow{#1}}
                  {\xRightarrow{\raisebox{-1.5pt}[0pt][0pt]{$\scriptstyle#1$}}}
                  {\xRightarrow{#1}}
                  {\xRightarrow{#1}}}{}
    \fi
  \fi  \if\relax\detokenize{#2}\relax\else^{#2}\fi  \if\relax\detokenize{#3}\relax\else_{#3}\fi}}
\newcommand{\raw@reduce}[3]{\mathrel{\if\relax\detokenize{#1}\relax
    \longrightarrow
  \else
    \setbox0=\hbox{$\scriptstyle#1$}\setlength{\@overset@width}{\wd0} 
    \ifdim\@overset@width<0.75em
      {\overset{#1\mkern4mu}{\Longrightarrow}}{}
    \else
      {\xrightarrow{#1}}{}
    \fi
  \fi  \if\relax\detokenize{#2}\relax\else^{#2}\fi  \if\relax\detokenize{#3}\relax\else_{#3}\fi}}

\newcommand{\xRrightarrow}[2][]{\ext@arrow 0359\Rrightarrowfill@{#1}{#2}}
\newcommand{\Rrightarrowfill@}{\arrowfill@\equiv\equiv\Rrightarrow}
\newcommand{\xLleftarrow}[2][]{\ext@arrow 3095\Lleftarrowfill@{#1}{#2}}
\newcommand{\Lleftarrowfill@}{\arrowfill@\Lleftarrow\equiv\equiv}

\def\rightarrowfill@script{\arrowfill@{\scriptstyle\relbar}{\scriptstyle\relbar}{\scriptstyle\rightarrow}}

\newcommand*\xrightrightarrows[2][]{\mathrel{  \raise.6ex\hbox{    $\ext@arrow 0359\rightarrowfill@script{\phantom{#1}}{#2}$}  \setbox0=\hbox{    $\ext@arrow 0359\rightarrowfill@script{#1}{\phantom{#2}}$}\kern-\wd0 \lower.2ex\box0}}

\newcommand{\raw@parstep}[3]{\mathrel{\if\relax\detokenize{#1}\relax
    \rightrightarrows
  \else
    \setbox0=\hbox{$\scriptstyle#1$}\setlength{\@overset@width}{\wd0} 
    \ifdim\@overset@width<0.75em
      {\overset{#1\mkern4mu}{\rightrightarrows}}{}
    \else
      {\xrightrightarrows{#1}}{}
    \fi
  \fi  \if\relax\detokenize{#2}\relax\else^{#2}\fi  \if\relax\detokenize{#3}\relax\else_{#3}\fi}}

\newcommand{\raw@bigstep}[3]{\mathrel{\if\relax\detokenize{#1}\relax
    \Rrightarrow
  \else
    \setbox0=\hbox{$\scriptstyle#1$}\setlength{\@overset@width}{\wd0} 
    \ifdim\@overset@width<0.75em
      {\overset{#1\mkern4mu}{\Rrightarrow}}{}
    \else
      {\xRrightarrow{#1}}{}
    \fi
  \fi  \if\relax\detokenize{#2}\relax\else^{#2}\fi  \if\relax\detokenize{#3}\relax\else_{#3}\fi}}

\newcommand{\step}[1][]{\raw@step{#1}{}{c}}
\newcommand{\stepsn}[2][]{\raw@step{#1}{#2}{c}}
\newcommand{\steps}[1]{\raw@step{#1}{*}{c}}
\newcommand{\stepss}[1][]{\raw@step{#1}{+}{c}}
\newcommand{\bigstep}[1][]{\raw@bigstep{#1}{}{c}}
\newcommand{\bigstepsn}[2][]{\raw@bigstep{#1}{#2}{c}}
\newcommand{\bigsteps}[1]{\raw@bigstep{#1}{*}{c}}
\newcommand{\bigstepss}[1]{\raw@bigstep{#1}{+}{c}}

\newcommand{\localstep}[1][]{\raw@reduce{#1}{}{}}
\newcommand{\localsteps}[1][]{\raw@reduce{#1}{*}{}}
\newcommand{\localstepss}[1][]{\raw@reduce{#1}{+}{}}

\newcommand{\ntwkstep}[1]{\raw@step{#1}{}{}}
\newcommand{\ntwksteps}[1]{\raw@step{#1}{*}{}}
\newcommand{\ntwkstepss}[1]{\raw@step{#1}{+}{}}
\newcommand{\ntwkparstep}[1]{\raw@parstep{#1}{}{}}
\newcommand{\ntwkparsteps}[1]{\raw@parstep{#1}{*}{}}
\newcommand{\ntwkbigstep}[1]{\raw@bigstep{#1}{}{}}
\newcommand{\ntwkbigsteps}[1]{\raw@bigstep{#1}{*}{}}

\newcommand{\systemstep}[1][]{\raw@step{#1}{}{S}}
\newcommand{\systemsteps}[1][]{\raw@step{#1}{*}{S}}
\newcommand{\systemstepsn}[2][]{\raw@step{#1}{#2}{S}}
\newcommand{\systemstepss}[1][]{\raw@step{#1}{+}{S}}
\newcommand{\systemparstep}[1]{\raw@parstep{#1}{}{S}}
\newcommand{\systemparsteps}[1]{\raw@parstep{#1}{*}{S}}
\newcommand{\systemparstepsn}[2][]{\raw@parstep{#1}{#2}{S}}
\newcommand{\systembigstep}[1]{\raw@bigstep{#1}{}{S}}
\newcommand{\systembigsteps}[1]{\raw@bigstep{#1}{*}{S}}
\newcommand{\systembigstepsn}[2][]{\raw@bigstep{#1}{#2}{S}}

\newcommand{\raw@nstep}[3]{\mathrel{\if\relax\detokenize{#1}\relax
    {\centernot{\Longrightarrow}}{}
  \else
    {\xnRightarrow{\minwidthbox{0.75em}{\ensuremath{\scriptstyle#1}}}}{}
  \fi  \if\relax\detokenize{#2}\relax\else^{#2}\fi  \if\relax\detokenize{#3}\relax\else_{#3}\fi}}
\newcommand{\nstep}[1]{\raw@nstep{#1}{}{c}}
\newcommand{\nlocalstep}[1][]{\raw@nstep{#1}{}{e}}
\makeatother

\newcommand{\trc}{t}

\newcommand\send[3]{#1 \ChorSend[#2] #3}

\newcommand{\TySepCol}[1]{\begingroup\color{chorcolor}{#1}\endgroup}
\newcommand{\LocalTySepCol}[1]{\begingroup\color{localcolor}{#1}\endgroup}

\newcommand\ctx{\Theta}

\newcommand\locs{\mathrel{\rhd}}
\newcommand\locsCol{\mathrel{\TySepCol{\locs}}}

\newcommand\forked{\mathrel{\rotatebox[origin=c]{90}{\raisebox{-0.8pt}{$\pitchfork$}}}}
\newcommand\forkedCol{\mathrel{\TySepCol{\forked}}}

\newcommand\provesCol{\colrel{chorcolor}{\proves}}
\newcommand\provesrevCol{\colrel{chorcolor}{\provesrev}}
\newcommand\provesPlusCol{\colrel{chorcolor}{\provesPlus}}
\newcommand\eprovesCol{\colrel{localcolor}{\eproves}}
\newcommand\tyCol{\colrel{chorcolor}{:}}
\newcommand\kndCol{\colrel{chorcolor}{::}}
\newcommand\etyCol{\colrel{localcolor}{:}}
\newcommand\ekndCol{\colrel{localcolor}{::}}
\newcommand\checkCol{\colrel{chorcolor}{\texttt{loc-ok}}}

\newcommand\localkinded[2]{\ensuremath{#1 \eprovesCol #2 \ekndCol *_e}}
\newcommand\localtyped[3]{\ensuremath{#1 \eprovesCol #2 \etyCol #3}}
\newcommand\localempkinded[1]{\localkinded{}{#1}}
\newcommand\localemptyped[2]{\ensuremath{\localtyped{}{#1}{#2}}}
\newcommand\localctxwf[2]{\ensuremath{#1 \eprovesCol #2}}

\definecolor{CheckColor}{HTML}{008F91}
\definecolor{SynthColor}{HTML}{922724}
\newcommand\checkarrow{\colrel{CheckColor}{\Downarrow}}
\newcommand\syntharrow{\colrel{SynthColor}{\Uparrow}}
\newcommand\botcheckarrow{\ensuremath{\adjustbox{trim=0pt 0pt 0pt 4.2pt, clip}{$\checkarrow$}}}
\newcommand\topsyntharrow{\ensuremath{\raisebox{2.5pt}{\adjustbox{trim=0pt 4.2pt 0pt 0pt, clip}{$\syntharrow$}}}}
\newcommand\checksyntharrow{\mathrel{\mathrlap{{\topsyntharrow}}{\botcheckarrow}}}

\newcommand\chorkinded[3]{\ensuremath{#1 \provesCol #2 \kndCol #3}}
\newcommand\chorempkinded[2]{\ensuremath{\, \provesCol #1 \kndCol #2}}
\newcommand\chortyped[4]{\ensuremath{#1 \provesCol #2 \tyCol #3 \locsCol #4}}
\newcommand\chortypedsynth[7]{\ensuremath{
  #1   \provesCol   #2 \ifthenelse{\equal{#3}{c}}{\checkarrow}{\syntharrow}
  #4 \ifthenelse{\equal{#5}{c}}{\checkarrow}{\syntharrow}
  #6 \provesrevCol
  #7
}}
\newcommand\chortypedsynthany[5]{\ensuremath{#1 \provesCol #2 \checksyntharrow #3 \checksyntharrow #4 \provesrevCol #5}}
\newcommand\chorsometyped[3]{\ensuremath{#1 \provesCol #2 \locsCol #3}}
\newcommand\choremptyped[3]{\ensuremath{\, \provesCol #1 \tyCol #2 \locsCol #3}}
\newcommand\chorctxwf[2]{\ensuremath{#1 \provesCol #2}}
\newcommand\chorempctxwf[1]{\ensuremath{\, \provesCol #1}}
\newcommand\chorwf[2][\ctx]{\ensuremath{{#1} \provesCol {#2} \checkCol}}
\newcommand\chorempwf[1]{\ensuremath{\, \provesCol {#1} \checkCol}}
\newcommand\chortypedplus[4]{\ensuremath{#1 \provesPlusCol #2 \tyCol #3 \locsCol #4}}
\newcommand\choremptypedplus[3]{\ensuremath{\, \provesPlusCol #1 \tyCol #2 \locsCol #3}}

\newcommand\localtypedcheck[3]{\ensuremath{#1 \eprovesCol #2 \checkarrow #3}}
\newcommand\localtypedsynth[3]{\ensuremath{#1 \eprovesCol #2 \syntharrow #3}}

\newcommand\wfSubst[4]{\ensuremath{#1 \provesCol #2 \tyCol #3 \mathrel{\TySepCol{\Rightarrow}} #4}}
\newcommand\wfChorSubst[5]{\ensuremath{#1 \provesCol #2 \tyCol #3 \mathrel{\TySepCol{\Rightarrow}} #4 \locsCol #5}}

\newcommand{\RDone}[3]{{#1}.({#2} \rightarrow {#3})}
\newcommand{\RArg}[1]{\FontChoreo{Arg}({#1})}
\newcommand{\RFun}[1]{\FontChoreo{Fun}({#1})}
\newcommand{\RPairL}[1]{\FontChoreo{PairL}({#1})}
\newcommand{\RPairR}[1]{\FontChoreo{PairR}({#1})}
\newcommand{\RApp}[1]{\FontChoreo{App}_{#1}}
\newcommand{\RSendV}[3]{{#1}.{#2} \ColSend {#3}}
\newcommand{\RIfTrue}[1]{\FontChoreo{if}_{#1}~\True}
\newcommand{\RIfFalse}[1]{\FontChoreo{if}_{#1}~\False}
\newcommand{\RTApp}[1]{\FontChoreo{TApp}_{#1}}
\newcommand{\RLet}[2]{\LetN~{#1} \ChorDef {#2}}
\newcommand{\RUnfoldFold}[1]{\FontChoreo{UnfoldFold}_{#1}}
\newcommand{\RFstPair}[1]{\FontChoreo{FstPair}_{#1}}
\newcommand{\RSndPair}[1]{\FontChoreo{SndPair}_{#1}}
\newcommand{\RCaseInl}[1]{\FontChoreo{CaseInl}_{#1}}
\newcommand{\RCaseInr}[1]{\FontChoreo{CaseInr}_{#1}}
\newcommand{\RLocalCaseInl}[1]{\FontChoreo{LocalCaseInl}_{#1}}
\newcommand{\RLocalCaseInr}[1]{\FontChoreo{LocalCaseInr}_{#1}}
\newcommand{\RFork}[2]{{#1}.\ForkN({#2})}
\newcommand{\RKill}[1]{\KillN({#1})}

\newcommand{\RRet}[2]{\Ret{{#1} \Rightarrow {#2}}}
\newcommand{\RArgNtwk}[1]{\FontNtwk{Arg}({#1})}
\newcommand{\RFunNtwk}[1]{\FontNtwk{Fun}({#1})}
\newcommand{\RPairLNtwk}[1]{\FontNtwk{PairL}({#1})}
\newcommand{\RPairRNtwk}[1]{\FontNtwk{PairR}({#1})}
\newcommand{\RSendNtwk}[2]{{#1} \NtwkSend {#2}}
\newcommand{\RRecvNtwk}[2]{{#1}.{#2} \NtwkSend}
\newcommand{\RAppNtwk}{\FontNtwk{App}}
\newcommand{\RIfTrueNtwk}{\FontNtwk{if}~\True}
\newcommand{\RIfFalseNtwk}{\FontNtwk{if}~\False}
\newcommand{\RTAppNtwk}{\FontNtwk{TApp}}
\newcommand{\RLetNtwk}[1]{\NtwkLetN\NtwkDef {#1}}
\newcommand{\RUnfoldFoldNtwk}{\FontNtwk{UnfoldFold}}
\newcommand{\RFstPairNtwk}{\FontNtwk{FstPair}}
\newcommand{\RSndPairNtwk}{\FontNtwk{SndPair}}
\newcommand{\RCaseInlNtwk}{\FontNtwk{CaseInl}}
\newcommand{\RCaseInrNtwk}{\FontNtwk{CaseInr}}
\newcommand{\RForkNtwk}[2]{\NtwkForkN({#1},{#2})}
\newcommand{\RExitNtwk}{\NtwkExit}

\newcommand{\RForkSys}[3]{{#1}.\SysForkN({#2},{#3})}
\newcommand{\RKillSys}[1]{\SysKillN({#1})}

\newcommand{\extract}[2]{\lfloor {#1} \rfloor_{#2}}

\newcommand{\cloc}[1]{\operatorname{cloc}({#1})}
\newcommand{\clocStrict}[1]{\operatorname{cloc'}({#1})}
\newcommand{\rloc}[1]{\operatorname{rloc}({#1})}
\newcommand{\tloc}[2][\ctx]{\operatorname{tloc}({#1};{#2})}
\newcommand{\loc}[1]{\operatorname{loc}({#1})}
\newcommand{\spawned}[1]{\operatorname{spawned}({#1})}
\newcommand{\ctxlabel}[1]{{#1}[l]}
\newcommand{\ctxredex}[1]{{#1}[R]}
\newcommand{\collapse}[1]{\operatorname{collapse}({#1})}

\newtcolorbox{mybox}[1][]{
    enhanced,
    breakable,
    title = {#1},
    sharpish corners,
    before skip=\baselineskip,
    leftupper=1.5cm,
    boxrule=0.5pt,
    top=15pt,
    colback=white,
    left=15pt
}


